Curriculum for Crowd Counting -- Is it Worthy?

Recent advances in deep learning techniques have achieved remarkable performance in several computer vision problems. A notably intuitive technique called Curriculum Learning (CL) has been introduced recently for training deep learning models. Surprisingly, curriculum learning achieves significantly improved results in some tasks but marginal or no improvement in others. Hence, there is still a debate about its adoption as a standard method to train supervised learning models. In this work, we investigate the impact of curriculum learning in crowd counting using the density estimation method. We performed detailed investigations by conducting 112 experiments using six different CL settings using eight different crowd models. Our experiments show that curriculum learning improves the model learning performance and shortens the convergence time.

==> tables/tab1_results1.tex <==



\begin{table*}
\centering
\caption{Performance evaluation of curriculum learning in different crowd counting models over ShanghaiTech Part A dataset.}
\begin{tabular}{ccccccccccccccc} \toprule
\multirow{2}{*}{Models} &\multicolumn{2}{c}{Without CL}
&\multicolumn{2}{c}{Linear} &\multicolumn{2}{c}{Quadratic} &\multicolumn{2}{c}{Root} &\multicolumn{2}{c}{Step} &\multicolumn{2}{c}{Exponential} &\multicolumn{2}{c}{CL parameters*} \\[0.5em] 
&MAE &MSE &MAE &MSE  &MAE &MSE &MAE &MSE &MAE &MSE &MAE &MSE  &a &b \\ \midrule  \midrule

MCNN \cite{MCNN_CVPR2016} & \cellcolor{c1}0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &a &b \\[0.5em]

CMTL  &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &a &b \\[0.5em]

MSCNN \cite{MSCNN_ICIP2017} &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &a &b \\[0.5em]

CSRNet \cite{CSRNet_CVPR2018} &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &a &b \\[0.5em]

SANet \cite{SANet_ECCV2018} &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &a &b \\[0.5em]

TEDnet \cite{TEDnet_CVPR2019} &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &a &b \\[0.5em]

Yang et al. \cite{} &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &a &b \\[0.5em]

SASNet \cite{SASNet_AAAI2021} &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &a &b \\[0.5em]

MAN \cite{} &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &a &b \\[0.5em]

\bottomrule
\end{tabular}
\end{table*}

